Climbing the cosmic ladder with stellar twins in RAVE with Gaia

We apply the twin method to determine parallaxes to 232,545 stars of the RAVE survey using the parallaxes of Gaia DR1 as a reference. To search for twins in this large dataset, we apply the t-stochastic neighbour embedding t-SNE projection which distributes the data according to their spectral morphology on a two dimensional map. From this map we choose the twin candidates for which we calculate a chi^2 to select the best sets of twins. Our results show a competitive performance when compared to other model-dependent methods relying on stellar parameters and isochrones. The power of the method is shown by finding that the accuracy of our results is not significantly affected if the stars are normal or peculiar since the method is model free. We find twins for 60% of the RAVE sample which is not contained in TGAS or that have TGAS uncertainties which are larger than 20%. We could determine parallaxes with typical errors of 28%. We provide a complementary dataset for the RAVE stars not covered by TGAS, or that have TGAS uncertainties which are larger than 20%, with model-free parallaxes scaled to the Gaia measurements.

==> individual_plx_cl_long.tex <==
\begin{tabular}{|l|l|r|r|r|}
\hline
  \multicolumn{1}{|c|}{cluster} &
  \multicolumn{1}{c|}{star} &
  \multicolumn{1}{c|}{twin\_plx} &
  \multicolumn{1}{c|}{e\_twin\_plx} &
  \multicolumn{1}{c|}{ntw} \\
\hline
  Blanco 1 & 20050807\_0005m26\_005 & 5.79238 & 0.132197 & 428\\
  Blanco 1 & 20060726\_2353m28\_122 & 3.29293 & 0.0547224 & 673\\
  Blanco 1 & 20060930\_2359m33\_084 & 3.057 & 0.0594117 & 613\\
  Blanco 1 & 20061118\_2353m28\_117 & 4.22382 & 0.249239 & 84\\
  Blanco 1 & 20061118\_2353m28\_118 & 3.49395 & 0.111179 & 265\\
  Blanco 1 & 20110727\_2353m28b\_116 & 5.37608 & 0.12647 & 467\\
  Blanco 1 & 20110905\_0020m31\_044 & 3.00227 & 0.10113 & 443\\
  Melotte 22 & 20120107\_0336p23\_107 & 5.6664 & 0.183508 & 252\\
  Melotte 22 & 20120107\_0336p23\_115 & 6.38786 & 0.208054 & 267\\
  Melotte 22 & 20120107\_0336p23\_119 & 6.35511 & 0.380769 & 39\\
  Melotte 22 & 20120109\_0346p23\_117 & 7.00413 & 0.282162 & 15\\
  Melotte 22 & 20120109\_0346p23\_127 & 5.68836 & 0.157212 & 366\\
  Melotte 22 & 20120109\_0346p23\_133 & 6.60906 & 0.334615 & 143\\
  Melotte 22 & 20120112\_0346p23\_117 & 6.44514 & 0.35437 & 17\\
  Melotte 22 & 20120112\_0346p23\_133 & 6.52762 & 0.348053 & 126\\
  NGC 2632 & 20120311\_0842p20\_070 & 4.28651 & 0.135522 & 304\\
  NGC 2632 & 20120311\_0842p20\_073 & 4.96664 & 0.208399 & 306\\
  NGC 2632 & 20120311\_0842p20\_081 & 5.4388 & 0.14661 & 348\\
  NGC 2632 & 20120311\_0842p20\_111 & 6.72983 & 0.141616 & 617\\
  NGC 2632 & 20120311\_0842p20\_136 & 4.11859 & 0.249014 & 72\\
  NGC 2632 & 20120313\_0842p20\_013 & 7.87249 & 0.118046 & 187\\
  NGC 2632 & 20120313\_0842p20\_017 & 5.35992 & 0.0938281 & 262\\
  NGC 2632 & 20120313\_0842p20\_029 & 5.48927 & 0.193961 & 281\\
  NGC 2632 & 20120313\_0842p20\_033 & 5.99426 & 0.119198 & 303\\
  NGC 2632 & 20120313\_0842p20\_039 & 5.77355 & 0.13513 & 278\\
  NGC 2632 & 20120313\_0842p20\_043 & 5.17471 & 0.14604 & 459\\
  NGC 2632 & 20120313\_0842p20\_047 & 5.67578 & 0.179691 & 238\\
  NGC 2632 & 20120313\_0842p20\_053 & 4.46148 & 0.284384 & 235\\
  NGC 2632 & 20120313\_0842p20\_057 & 5.63709 & 0.179007 & 289\\
  NGC 2632 & 20120313\_0842p20\_060 & 5.33806 & 0.266695 & 213\\
  NGC 2632 & 20120313\_0842p20\_100 & 7.12502 & 0.310122 & 209\\
  NGC 2632 & 20120313\_0842p20\_110 & 5.73823 & 0.239751 & 230\\
  NGC 2632 & 20120315\_0842p20\_027 & 5.01006 & 0.131977 & 549\\
  NGC 2632 & 20120315\_0842p20\_060 & 5.12125 & 0.0813797 & 877\\
  NGC 2682 & 20070409\_0851p11\_072 & 1.45839 & 0.0742917 & 97\\
  NGC 2682 & 20070409\_0851p11\_091 & 1.478 & 0.0794106 & 75\\
  NGC 2682 & 20070409\_0851p11\_105 & 0.963164 & 0.0584652 & 194\\
  NGC 2682 & 20070409\_0851p11\_120 & 1.38616 & 0.0594637 & 117\\
  NGC 2682 & 20070409\_0851p11\_137 & 1.21846 & 0.048161 & 83\\
  NGC 2682 & 20070409\_0851p11\_143 & 1.49361 & 0.150733 & 36\\
  NGC 2682 & 20070409\_0851p11\_146 & 0.904619 & 0.0367541 & 138\\
  NGC 2682 & 20070601\_0851p11\_101 & 2.07981 & 0.174662 & 97\\
  NGC 2682 & 20120411\_0850p11\_059 & 1.4601 & 0.032366 & 444\\
  NGC 2682 & 20120411\_0850p11\_094 & 1.48246 & 0.0474501 & 245\\
  NGC 2682 & 20120412\_0850p11\_042 & 1.51381 & 0.0326273 & 623\\
  NGC 2682 & 20120412\_0850p11\_103 & 1.83917 & 0.0852932 & 219\\
  NGC 2682 & 20120413\_0850p11\_042 & 1.29612 & 0.04869 & 239\\
  NGC 2682 & 20120511\_0850p11\_138 & 1.43756 & 0.162641 & 65\\
  IC 4651 & 20111004\_1725m49\_062 & 1.51702 & 0.0501477 & 169\\
  IC 4651 & 20111018\_1725m49\_049 & 1.21728 & 0.0390483 & 243\\
  IC 4651 & 20111018\_1725m49\_142 & 1.21914 & 0.0355467 & 198\\
  IC 4651 & 20111019\_1725m49\_039 & 1.6869 & 0.246843 & 36\\
  IC 4651 & 20111019\_1725m49\_113 & 1.6588 & 0.125771 & 47\\
  IC 4651 & 20111022\_1725m49\_022 & 1.83716 & 0.13872 & 68\\
  IC 4651 & 20111024\_1725m49\_091 & 2.05064 & 0.235572 & 80\\
  NGC 2422 & 20041123\_0739m14\_014 & 1.10875 & 0.0836123 & 21\\
  NGC 2422 & 20041123\_0739m14\_029 & 1.5233 & 0.0423619 & 320\\
  NGC 2422 & 20041123\_0739m14\_032 & 1.381 & 0.143923 & 33\\
  NGC 2422 & 20041130\_0739m14\_074 & 1.90669 & 0.0971225 & 72\\
  NGC 2477 & 20070214\_0746m39\_109 & 0.764643 & 0.0756366 & 66\\
  NGC 2477 & 20070327\_0746m39\_095 & 0.747429 & 0.0623176 & 21\\
  NGC 2477 & 20080327\_0746m39\_108 & 1.4805 & 0.104005 & 21\\
  NGC 2477 & 20080405\_0746m39\_116 & 1.75877 & 0.0838401 & 280\\
  NGC 2477 & 20090329\_0746m39\_086 & 0.912061 & 0.0480014 & 83\\
  NGC 2477 & 20091203\_0746m39\_107 & 1.10703 & 0.0593611 & 84\\
  NGC 2477 & 20091219\_0746m39\_091 & 0.741381 & 0.101944 & 54\\
  NGC 2477 & 20091219\_0746m39\_093 & 1.20627 & 0.207089 & 76\\
  NGC 2477 & 20091219\_0746m39\_099 & 0.776083 & 0.0204768 & 220\\
  NGC 2477 & 20110324\_0746m39\_095 & 0.923093 & 0.0519996 & 126\\
  NGC 2477 & 20110324\_0746m39\_108 & 0.767217 & 0.0512236 & 64\\
  NGC 2477 & 20120317\_0746m39\_106 & 1.26954 & 0.123299 & 93\\
  NGC 2477 & 20130110\_0752m38\_127 & 0.840882 & 0.0610065 & 48\\
  NGC 2477 & 20130110\_0752m38\_139 & 0.8485 & 0.0486678 & 29\\
  Hyades & 20111126\_0428p15\_035 & 21.0907 & 0.371738 & 278\\
  Hyades & 20111126\_0428p15\_078 & 22.127 & 0.373372 & 342\\
  Hyades & 20111126\_0428p15\_126 & 20.9253 & 0.427689 & 222\\
  Hyades & 20111201\_0430p15\_039 & 25.6331 & 0.542753 & 378\\
  Hyades & 20111201\_0430p15\_061 & 24.9866 & 0.926956 & 246\\
  Hyades & 20111201\_0430p15\_085 & 27.4549 & 0.261058 & 424\\
\hline\end{tabular}

